Conditional diffusions for amortized neural posterior estimation

Neural posterior estimation (NPE), a simulation-based computational approach for Bayesian inference, has shown great success in approximating complex posterior distributions. Existing NPE methods typically rely on normalizing flows, which approximate a distribution by composing many simple, invertible transformations. But flow-based models, while state of the art for NPE, are known to suffer from several limitations, including training instability and sharp trade-offs between representational power and computational cost. In this work, we demonstrate the effectiveness of conditional diffusions coupled with high-capacity summary networks for amortized NPE. Conditional diffusions address many of the challenges faced by flow-based methods. Our results show that, across a highly varied suite of benchmarking problems for NPE architectures, diffusions offer improved stability, superior accuracy, and faster training times, even with simpler, shallower models. Building on prior work on diffusions for NPE, we show that these gains persist across a variety of different summary network architectures. Code is available at https://github.com/TianyuCodings/cDiff.

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes/No/Not Applicable].

Yes. The mathematical setting is described throughout the paper, and the assumptions are formalized in Assumption \ref{assump:sufficiency}. The training and sampling procedures are outlined in Algorithm \ref{alg:train_cdiff} and Algorithm \ref{alg:sample_cdiff}, respectively. Detailed descriptions of the network structure and training strategies can be found in Appendix \ref{sec:diff_training} and Appendix \ref{sec:summary_network}.


\item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes/No/Not Applicable]

Yes. We measure the computation time and model size of our method and baseline models in Section \ref{sec:results}.


   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes/No/Not Applicable]

   No, we have not submitted the source code. However, we will make it publicly available after acceptance.
   
 \end{enumerate}




 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes/No/Not Applicable]

   Yes.
   
   \item Complete proofs of all theoretical results. [Yes/No/Not Applicable]

   Yes. The complete proof is provided in Appendix \ref{sec:diff_proof} and Appendix \ref{sec:summary_diffusion}.

   
   \item Clear explanations of any assumptions. [Yes/No/Not Applicable]    
   
   Yes, the explanations of the assumptions are provided immediately following each assumption statement.
   
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes/No/Not Applicable]

    No, we did not submit any code to replicate the figures and main experimental results along with the paper, but we will make it publicly available after acceptance.

   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes/No/Not Applicable]

    Yes, all training details are thoroughly described in Appendix \ref{sec:diff_training} and Appendix \ref{sec:summary_network}.

   
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes/No/Not Applicable]

    Yes, we have run our experiments 10 times with different random seeds, and the results reported in Table \ref{tab:benchmark_results} are the means of all runs.
    
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes/No/Not Applicable]

    Yes. The equipment details are provided in Section \ref{sec:results}.

 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
 
   \item Citations of the creator If your work uses existing assets. [Yes/No/Not Applicable]

    Not Applicable. We don't use any assets.
   
   \item The license information of the assets, if applicable. [Yes/No/Not Applicable]

Not Applicable. We don't use any assets.
    
   
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes/No/Not Applicable]

No. We do not provide access to our new assets at this stage. The assets will be made publicly available once the paper is accepted for publication.
   
   \item Information about consent from data providers/curators. [Yes/No/Not Applicable]

Not Applicable. No data provided outside.
   
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Yes/No/Not Applicable]

Not Applicable.
   
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Yes/No/Not Applicable]

Not Applicable.
   
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Yes/No/Not Applicable]

Not Applicable.

   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Yes/No/Not Applicable]

Not Applicable.

 \end{enumerate}

 \end{enumerate}
 
